Exploring the Viability of Synthetic Audio Data for Audio-Based Dialogue State Tracking

Dialogue state tracking plays a crucial role in extracting information in task-oriented dialogue systems. However, preceding research are limited to textual modalities, primarily due to the shortage of authentic human audio datasets. We address this by investigating synthetic audio data for audio-based DST. To this end, we develop cascading and end-to-end models, train them with our synthetic audio dataset, and test them on actual human speech data. To facilitate evaluation tailored to audio modalities, we introduce a novel PhonemeF1 to capture pronunciation similarity. Experimental results showed that models trained solely on synthetic datasets can generalize their performance to human voice data. By eliminating the dependency on human speech data collection, these insights pave the way for significant practical advancements in audio-based DST. Data and code are available at https://github.com/JihyunLee1/E2E-DST.

==> temp.tex/JGA_version.tex <==
\begin{table}[h]
\centering
\caption{Cascading (Cas.) and E2E performance comparison on SynthWOZ synthetic and human datasets.}
\label{tab:main}
\scalebox{0.93}{
\begin{tabular}{cl|lll}
\hline
\multicolumn{1}{l}{Model} & TestSet    & JGA     & F1     & PhonemeF1 \\\hline
\multirow{2}{*}{Cas.}      & Human & 13.46 & \textbf{62.07} & \textbf{76.79}     \\
                          & \small{Synth} 
                        & \footnotesize{21.49 \scriptsize{($\triangle$8.03)}}
                        & \footnotesize{71.32 \scriptsize{($\triangle$9.25)}}
                        & \footnotesize{81.51 \scriptsize{($\triangle$4.72)}}     \\\hline
\multirow{2}{*}{E2E}      & Human & \textbf{16.40}  & 61.99 & 76.28     \\
                          & \small{Synth} 
                          & \footnotesize{22.78 \scriptsize{($\triangle$6.38)}}
                          & \footnotesize{69.06 \scriptsize{($\triangle$7.07)}}
                          & \footnotesize{78.58 \scriptsize{($\triangle$2.30)}}     \\\hline
\end{tabular}
}
\end{table}
















\begin{table}[]
\centering

\caption{Generalizability between multi-speaker and single speaker datasets.}
\scalebox{0.93}{
\begin{tabular}{ll|lll}

\hline
Speaker & TestSet & JGA      & F1     & PhonemeF1      \\ \hline
\multirow{2}{*}{Single}  & Human   & 10.51   & 51.88 & 67.44         \\
                        & Synth   
                        &  \footnotesize{22.41 \scriptsize{($\triangle$2.30)}}  
                        & \footnotesize{67.53 \scriptsize{($\triangle$2.30)}}  
                        & \footnotesize{76.48 \scriptsize{($\triangle$2.30)}}         \\ \hline
\multirow{2}{*}{Multi}   & Human   & \textbf{16.40}   & \textbf{61.99} & \textbf{76.28}         \\
                            & Synth   
                            & \footnotesize{22.78 \scriptsize{($\triangle$2.30)}}    
                            & \footnotesize{69.06 \scriptsize{($\triangle$2.30)}} 
                            & \footnotesize{78.58 \scriptsize{($\triangle$2.30)}}         \\\hline
\end{tabular}
}
\label{tab:single_speaker}
\end{table}


















\begin{table}[]
\centering
\caption{Effect of contextual information on JGA, joint slot-value (F1), and Slot-F1 accuracies. \textit{U}: user, \textit{S}:system.}
\resizebox{\columnwidth}{!}{
\begin{tabular}{cl|l|lll}
\hline
\multicolumn{2}{c|}{Model}                                       & Test-set & \multicolumn{1}{c}{JGA} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{PhonemeF1} \\ \hline
\multicolumn{1}{c|}{\multirow{4}{*}{\rotatebox[origin=c]{90}{ Cas. }}} & \multirow{2}{*}{\small{U}}   
& Human    & 8.35                  & 52.16                 & 68.33                  \\
\multicolumn{1}{c|}{}                     &                      
& Synth    
& \footnotesize{19.25 \scriptsize{($\triangle$-)}}                
& \footnotesize{67.97 \scriptsize{($\triangle$-)}}                 
& \footnotesize{78.45 \scriptsize{($\triangle$-)}}                     \\ \cline{3-6} 
\multicolumn{1}{c|}{}                     & \multirow{2}{*}{\small{U+S} }
& Human    & 13.46                  & 62.07                  & 76.79                     \\
\multicolumn{1}{c|}{}                     &                      
& Synth    
& \footnotesize{21.49 \scriptsize{($\triangle$2.30)}}                  
& \footnotesize{71.32 \scriptsize{($\triangle$2.30)}}                 
& \footnotesize{81.51\scriptsize{($\triangle$2.30)}}                     \\ \hline\hline
\multicolumn{1}{c|}{\multirow{4}{*}{\rotatebox[origin=c]{90}{ E2E }}} & \multirow{2}{*}{\small{U}}   
& Human    & 12.77                 & 56.84                & 69.51                    \\
\multicolumn{1}{c|}{}                     &                      
& Synth    
& \footnotesize{20.56 \scriptsize{($\triangle$-)}}                  
& \footnotesize{64.08 \scriptsize{($\triangle$-)}}                 
& \footnotesize{74.47 \scriptsize{($\triangle$-)}}                     \\ \cline{3-6} 
\multicolumn{1}{c|}{}                     & \multirow{2}{*}{\small{U+S}} 
& Human    & \textbf{16.40}                   & \textbf{61.99}                 & \textbf{76.28}                     \\
\multicolumn{1}{c|}{}                     &                      
& Synth    
& \footnotesize{22.78 \scriptsize{($\triangle$2.30)}}                 
& \footnotesize{69.06 \scriptsize{($\triangle$2.30)}}                 
& \footnotesize{78.58 \scriptsize{($\triangle$2.30)}}                       \\ \hline
\end{tabular}
}
\label{tab:tab:with_sys}
\end{table}


==> temp.tex/tables.tex <==
% \begin{table}[]
% \resizebox{\columnwidth}{!}{
% \small{
% \begin{tabular}{ll|p{14.5mm}p{14.5mm}p{14.5mm}p{14.5mm}}
% \hline
% \multicolumn{2}{l|}{\textbf{Model}}                                 & \multicolumn{1}{p{12mm}}{\textbf{Name \newline \footnotesize{(40.8\%)}}} & \multicolumn{1}{p{12mm}}{\textbf{Cat. \footnotesize{(33.25\%)}}} & \multicolumn{1}{p{12mm}}{\textbf{Number \footnotesize{(16.1\%)}}} & \multicolumn{1}{p{11mm}}{\textbf{Time \footnotesize{(9.8\%)}}} \\ \hline
% \multicolumn{1}{l|}{\multirow{2}{*}{\rotatebox[origin=c]{90}{ Cas. }}} & \textbf{Hum.} & 42.04                                      & 50.39                                       & 39.43                                        & 43.52                                     \\
% \multicolumn{1}{l|}{}                              & \textbf{\small{Synth} } & \footnotesize{54.21 \scriptsize{($\triangle$2.3)}}                                      & \footnotesize{55.37 \scriptsize{($\triangle$2.3)}}                                       & \footnotesize{51.88 \scriptsize{($\triangle$2.3)}}                                        & \footnotesize{54.22 \scriptsize{($\triangle$2.3)}}                                     \\\hline
% \multicolumn{1}{l|}{\multirow{2}{*}{\rotatebox[origin=c]{90}{ E2E }}} & \textbf{Hum.} & 34.61                                      & 59.56                                       & 40.54                                        & 42.22                                     \\
% \multicolumn{1}{l|}{}                              & \textbf{\small{Synth} } & \footnotesize{40.91 \scriptsize{($\triangle$2.3)}}                                      & \footnotesize{61.31 \scriptsize{($\triangle$2.3)}}                                       & \footnotesize{46.13 \scriptsize{($\triangle$2.3)}}                                        & \footnotesize{50.40 \scriptsize{($\triangle$2.3)}} \\
% \hline
% \end{tabular}
% }
% }
% \end{table}


% \begin{table}[h]
% \label{tab:err_type}
% \centering
% \caption{Error classification on answer predictions.}
% \label{tab:main}
% \scalebox{0.84}{
% \begin{tabular}{l|l|lll}
% \hline
% \textbf{Model}                & \textbf{TestSet} & \textbf{Type1 \scriptsize{(Wrong)}} & \textbf{Type2 \scriptsize{((Ignore)}} & \textbf{Type3 \scriptsize{(Spurios)}} \\ \hline
% \multirow{2}{*}{Cas.} & Human  & 1000\scriptsize{28.74\%} & 1936\scriptsize{55.65\%} & 543\scriptsize{15.61\%} \\
%                      & \small{Synth}  
%                      & \footnotesize{25.70\%} \scriptsize{($\triangle$2.30)}
%                      & \footnotesize{63.26\%}\scriptsize{($\triangle$2.30)} 
%                      & \footnotesize{11.04\%}\scriptsize{($\triangle$2.30)} \\ \hline
% \multirow{2}{*}{E2E} & Human  & 24.54\% & 57.49\% & 17.97\% \\
%                      & \small{Synth}  
%                      & \footnotesize{20.14\%} \scriptsize{($\triangle$2.30)}
%                      & \footnotesize{61.70\%} \scriptsize{($\triangle$2.30)}
%                      & \footnotesize{18.16\%} \scriptsize{($\triangle$2.30)} \\ \hline
% % \multicolumn{2}{l|}{CSS \cite{Analysis-css}}      & \multicolumn{1}{l}{23.15\% } & \multicolumn{1}{l}{43.35\% } & \multicolumn{1}{l}{33.5\% } \\
% % \multicolumn{2}{l|}{STARC \cite{Analysis-QA-few}}    & \multicolumn{1}{l}{30.6\% }  & \multicolumn{1}{l}{43.7\% }  & \multicolumn{1}{l}{25.6\% } \\ \hline
% \end{tabular}
% }

% \end{table}

% \begin{table}[h]

% \centering

% \scalebox{0.98}{
% \begin{tabular}{c|c|l|l|l}
% \hline
% \multicolumn{1}{l|}{\textbf{Model}} & \textbf{Type} & \multicolumn{1}{c|}{\textbf{Ground}} & \multicolumn{1}{c|}{\textbf{Pred.}} & \multicolumn{1}{c}{\textbf{Ratio}} \\ \hline
% \multirow{3}{*}{\textbf{Cas.}}     & 1                   & Active                               & Active                              & 0.302                              \\
%                                     & 2                   & Active                               & None                                & 0.121                              \\
%                                     & 3                   & None                                 & Active                              & 0.576                              \\ \hline
% \multirow{3}{*}{\textbf{E2E}}       & 1                   & Active                               & Active                              & 0.245                              \\
%                                     & 2                   & Active                               & None                                & 0.180                              \\
%                                     & 3                   & None                                 & Active                              & 0.575                              \\ \hline

% \end{tabular}}

% \end{table}




% \begin{table}[t]
% \centering
% \caption{Gold, cascading and E2E performance comparison on SynthWOZ synthetic and human datasets.}
% \label{tab:main}
% \resizebox{\columnwidth}{!}{{\begin{tabular}{ll|cc|cc}
% \hline
% \multicolumn{2}{l|}{\multirow{2}{*}{Models}} &
%   \multicolumn{2}{c|}{Test-Synth} &
%   \multicolumn{2}{c}{Test-Human} \\ \cline{3-6} 
% \multicolumn{2}{l|}{} &
%   \multicolumn{1}{l|}{F1} &

%   \multicolumn{1}{l|}{Phoneme-F1} &
%   \multicolumn{1}{l|}{F1} &

%   \multicolumn{1}{l}{Phoneme-F1} \\ \hline
% \multicolumn{2}{l|}{Gold $\rightarrow$  Bart} & 
%   \multicolumn{1}{c|}{0.730} &

%   0.815 &
%   \multicolumn{1}{c|}{0.722} &

%   0.806 \\ \hline\hline
% \multicolumn{1}{l|}{\multirow{2}{*}{Casc. }} &
%   W2V w/ CTC $\rightarrow$ Bart &
%   \multicolumn{1}{c|}{\textbf{0.719}} &

%   \textbf{0.813} &
%   \multicolumn{1}{c|}{0.625} &

%   0.768 \\
% \multicolumn{1}{l|}{} &
%   Whisper $\rightarrow$  Bart &
%   \multicolumn{1}{c|}{0.708} &

%   0.793 &
%   \multicolumn{1}{c|}{\textbf{0.691}} &

%   \textbf{0.805} \\ \cline{1-2}
% \multicolumn{1}{l|}{E2E} &
%   W2V w/ Bart &
%   \multicolumn{1}{c|}{0.691} &

%   0.778 &
%   \multicolumn{1}{c|}{0.620} &

%   0.753 \\ \hline
% \end{tabular}}
% }
% \end{table}

% \begin{table}[t]
% \centering
% \caption{Cascading (Cas.) and E2E performance comparison on SynthWOZ synthetic and human datasets.}
% \label{tab:main}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{ll|lcc|lcc}
% \hline
% \multicolumn{2}{l|}{\multirow{2}{*}{Models}} & \multicolumn{3}{c|}{Test-Synth} & \multicolumn{3}{c}{Test-Human}\\ \cline{3-8} 
% \multicolumn{2}{l|}{}  & \multicolumn{1}{l|}{JGA}  & \multicolumn{1}{l|}{F1}    & \multicolumn{1}{l|}{Phoneme-F1} & \multicolumn{1}{l|}{JGA}  & \multicolumn{1}{l|}{F1}    & \multicolumn{1}{l}{Phoneme-F1}  \\ \hline
% \multicolumn{1}{l|}{\multirow{2}{*}{\rotatebox[origin=c]{90}{ Cas. }}} & W2V w/ CTC $\rightarrow$ Bart & \multicolumn{1}{l|}{0.2149} & \multicolumn{1}{c|}{0.7132} & 0.8151 & \multicolumn{1}{l|}{0.1346} & \multicolumn{1}{c|}{0.6207} & 0.7679   \\
% \multicolumn{1}{l|}{} & Whisper $\rightarrow$  Bart   & \multicolumn{1}{l|}{0.2207} & \multicolumn{1}{c|}{\textbf{0.7264}} & \textbf{0.8154}  & \multicolumn{1}{l|}{\textbf{0.1660}}  & \multicolumn{1}{c|}{\textbf{0.6788}} & \textbf{0.8160} \\ \cline{1-2}
% \multicolumn{1}{l|}{\rotatebox[origin=c]{90}{ E2E }} & W2V w/ Bart  & \multicolumn{1}{l|}{\textbf{0.2278}} & \multicolumn{1}{c|}{0.6906} & 0.7858   & \multicolumn{1}{l|}{0.1640} & \multicolumn{1}{c|}{0.6199} & 0.7628  \\ \hline
% \end{tabular}}
% \end{table}
% two cascading


% Therefore, demonstrates successful state tracking on both the synthesized and human speech testsets.

% lexical

% \begin{table}[t]
% \centering
% \caption{Effect of contextual information on Slot-F1 and joint slot-value (F1) accuracies.}
% \resizebox{\columnwidth}{!}{%
% \label{tab:user_only}
% \begin{tabular}{cl|l|ll|ll}
% \hline
% \multicolumn{2}{c|}{\multirow{2}{*}{\textbf{Model}}}                                      & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Data}}} & \multicolumn{2}{c|}{\textbf{Test-Synth}} & \multicolumn{2}{c}{\textbf{Test-Human}} \\ \cline{4-7} 
% \multicolumn{2}{c|}{}                                                                     & \multicolumn{1}{c|}{}                               & \multicolumn{1}{l|}{Slot-F1}   & F1      & \multicolumn{1}{l|}{Slot-F1}   & F1     \\ \hline 
% \multicolumn{2}{c|}{\multirow{2}{*}{Gold $\rightarrow$ Bart}}                                & user                                                & \multicolumn{1}{l|}{0.799}     & 0.703   & \multicolumn{1}{l|}{0.804}     & 0.715  \\
% \multicolumn{2}{c|}{}                                                                     & user + sys                                          & \multicolumn{1}{l|}{\textbf{0.819}}     & \textbf{0.730}   & \multicolumn{1}{l|}{\textbf{0.816}}     & \textbf{0.721}  \\ \hline\hline
% \multicolumn{1}{c|}{\multirow{4}{*}{\textbf{Casc.}}} & \multirow{2}{*}{W2V w/ CTC $\rightarrow$ Bart} & user                                                & \multicolumn{1}{l|}{0.788}     & 0.693   & \multicolumn{1}{l|}{0.726}     & 0.593  \\
% \multicolumn{1}{c|}{}                                &                                    & user + sys                                          & \multicolumn{1}{l|}{\textbf{0.817}}     & \textbf{0.719}   & \multicolumn{1}{l|}{\textbf{0.777}}     & \textbf{0.624}  \\\cline{2-7}
% \multicolumn{1}{c|}{}                                & \multirow{2}{*}{Whisper $\rightarrow$ Bart}    & user                                                & \multicolumn{1}{l|}{0.773}     & 0.694   & \multicolumn{1}{l|}{0.772}     & 0.652  \\
% \multicolumn{1}{c|}{}                                &                                    & user + sys                                          & \multicolumn{1}{l|}{\textbf{0.794}}     & \textbf{0.708}   & \multicolumn{1}{l|}{\textbf{0.813}}     & \textbf{0.690}  \\ \hline
% \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{E2E}}}   & \multirow{2}{*}{W2V w/ Bart}       & user                                                & \multicolumn{1}{l|}{0.749}     & 0.641   & \multicolumn{1}{l|}{0.702}     & 0.568  \\
% \multicolumn{1}{c|}{}                                &                                    & user + sys                                          & \multicolumn{1}{l|}{\textbf{0.790}}     & \textbf{0.691}   & \multicolumn{1}{l|}{\textbf{0.771}}     & \textbf{0.619}  \\ \hline
% \end{tabular}}
% \label{tab:with_sys}
% \end{table}

% \begin{table}[t]
% \centering
% \caption{Effect of contextual information on JGA, joint slot-value (F1), and Slot-F1 accuracies. \textit{U}: user, \textit{S}:system.}
% \resizebox{\columnwidth}{!}{%
% \label{tab:user_only}
% \begin{tabular}{cl|l|l|l|lll}
% \hline
% \multicolumn{2}{c|}{\multirow{2}{*}{Model}}  & \multicolumn{1}{c|}{\multirow{2}{*}{Data}} & \multicolumn{3}{c|}{Test-Synth}  & \multicolumn{3}{c}{Test-Human}   \\ \cline{4-9} 
% \multicolumn{2}{c|}{} & \multicolumn{1}{c|}{} & JGA  & \multicolumn{1}{c|}{F1} & Slot-F1 & \multicolumn{1}{l|}{JGA}  & \multicolumn{1}{c|}{F1}    & Slot-F1 \\ \hline
% \multicolumn{1}{c|}{\multirow{2}{*}{\rotatebox[origin=c]{90}{ Cas. }}} & \multirow{2}{*}{W2V w/ CTC $\rightarrow$ Bart}    & 0.1925 & 0.6797  & 0.7911   & \multicolumn{1}{l|}{0.0835} & \multicolumn{1}{l|}{0.5216} & 0.6936   \\
% \multicolumn{1}{c|}{} &   & \textbf{0.2149} & \textbf{0.7132}  & \textbf{0.8212}   & \multicolumn{1}{l|}{\textbf{0.1346}} & \multicolumn{1}{l|}{\textbf{0.6207}} & \textbf{0.7773}   \\ \cline{2-9} 

% \multicolumn{1}{c|}{\multirow{2}{*}{\rotatebox[origin=c]{90}{E2E}}}   & \multirow{2}{*}{W2V w/ Bart}                    & 0.2056 & 0.6408   & 0.7498   & \multicolumn{1}{l|}{0.1277} & \multicolumn{1}{l|}{0.5684} & 0.7021   \\
% \multicolumn{1}{c|}{}   &  & \textbf{0.2278} & \textbf{0.6906}   & \textbf{0.7900}  & \multicolumn{1}{l|}{\textbf{0.1640}} & \multicolumn{1}{l|}{\textbf{0.6199}} & \textbf{0.7711}   \\ \hline
% \end{tabular}}
% \label{tab:with_sys}
% \end{table}


\begin{table}[t]
\centering
\caption{Effect of contextual information on JGA, joint slot-value (F1), and Slot-F1 accuracies. \textit{U}: user, \textit{S}:system.}
\resizebox{\columnwidth}{!}{%
\label{tab:user_only}
\begin{tabular}{cl|l|l|l|l|lll}
\hline
\multicolumn{2}{c|}{\multirow{2}{*}{Model}}  & \multicolumn{1}{c|}{\multirow{2}{*}{Data}} & \multicolumn{3}{c|}{Test-Synth}  & \multicolumn{3}{c}{Test-Human}   \\ \cline{4-9} 
\multicolumn{2}{c|}{} & \multicolumn{1}{c|}{} & JGA  & \multicolumn{1}{c|}{F1} & Slot-F1 & \multicolumn{1}{l|}{JGA}  & \multicolumn{1}{c|}{F1}    & Slot-F1 \\ \hline
\multicolumn{1}{c|}{\multirow{4}{*}{\rotatebox[origin=c]{90}{ Cas. }}} & \multirow{2}{*}{W2V w/ CTC $\rightarrow$ Bart} & U   & 0.1925 & 0.6797  & 0.7911   & \multicolumn{1}{l|}{0.0835} & \multicolumn{1}{l|}{0.5216} & 0.6936   \\
\multicolumn{1}{c|}{} &  & U+S  & \textbf{0.2149} & \textbf{0.7132}  & \textbf{0.8212}   & \multicolumn{1}{l|}{\textbf{0.1346}} & \multicolumn{1}{l|}{\textbf{0.6207}} & \textbf{0.7773}   \\ \cline{2-9} 
\multicolumn{1}{c|}{}  & \multirow{2}{*}{Whisper $\rightarrow$ Bart}  & U  & 0.1662  & 0.6815  & 0.7685   & \multicolumn{1}{l|}{0.1415}   & \multicolumn{1}{l|}{0.6226} & 0.7878   \\
\multicolumn{1}{c|}{}    &       & U+S     & \textbf{0.2207}  &\textbf{0.7264}  & \textbf{0.8211}   & \multicolumn{1}{l|}{\textbf{0.1660}}  & \multicolumn{1}{l|}{\textbf{0.6787}} & \textbf{0.8262}   \\ \hline
\multicolumn{1}{c|}{\multirow{2}{*}{\rotatebox[origin=c]{90}{E2E}}}   & \multirow{2}{*}{W2V w/ Bart}                   & U  & 0.2056 & 0.6408   & 0.7498   & \multicolumn{1}{l|}{0.1277} & \multicolumn{1}{l|}{0.5684} & 0.7021   \\
\multicolumn{1}{c|}{}   &  & U+S & \textbf{0.2278} & \textbf{0.6906}   & \textbf{0.7900}  & \multicolumn{1}{l|}{\textbf{0.1640}} & \multicolumn{1}{l|}{\textbf{0.6199}} & \textbf{0.7711}   \\ \hline
\end{tabular}}
\label{tab:with_sys}
\end{table}


\begin{table}[]
\centering

\caption{Generalizability between multispeaker and single speaker datasets.}

\scalebox{0.80}{
\begin{tabular}{cc|l|cc}
\hline
\multicolumn{2}{c|}{\textbf{Model}}  & \textbf{Speaker}    & \multicolumn{1}{l}{\textbf{Test-Synth}} & \multicolumn{1}{l}{\textbf{Test-Human}} \\ \hline
\multicolumn{1}{l|}{\multirow{2}{*}{\textbf{E2E}}} & \multirow{2}{*}{W2V w/ Bart} & Single     & 0.6753  & 0.5188    \\ 
\multicolumn{1}{l|}{}  &      & Multi  & \textbf{0.6906}  & \textbf{0.6199}                          \\ \hline
\end{tabular}
}
\label{tab:single_speaker}

\end{table}



\begin{table}[t]


\centering
\caption{Quantitative comparison of different speech-based datasets. \textit{Ours-S}: Synthetic, \textit{Ours-H}: Human Speech.}
% \scalebox{0.76}{
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|c|l|l|l|l}
\hline
\multicolumn{1}{c|}{\textbf{}} & \multicolumn{1}{l|}{\textbf{FSC}} & \textbf{Snips} & \textbf{SLURP} & \textbf{Ours-S}    & \textbf{Ours-H} \\ \hline
Audio Files                    & 30,043                            & 5,886          & 72,277         & \textbf{142,850} & \textbf{1,018}                        \\
Duration {[}hrs{]}             & 19                                & 5.5            & 58             & \textbf{147.8}   & \textbf{1.27}                        \\
Avg. length {[}s{]}            & 2.3                               & 3.4            & 2.9            & \textbf{3.7}     & \textbf{4.5}    \\
\hline
\end{tabular}
}
\label{tab:data_audio}
\end{table}

\begin{table}[t]
\label{tab:data_lexical}

\centering
\caption{Lexical analysis of different speech-based datasets. \textit{Ours-S}: Synthetic, \textit{Ours-H}: Human speech.}
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|l|l|l|l|l}
\hline
& \textbf{FSC} & \textbf{SNIPS} & \textbf{SLURP} & \textbf{Ours-S} & \textbf{Ours-H} \\ \hline
                                          
\textbf{Avg. turns in dialogue}    & 1   & 1  & 1  & \textbf{13.45}  & \textbf{8.48}  \\
\textbf{Avg. turn spans per topic} & 1   & 1  & 1  & \textbf{2.37} & \textbf{2.14}    \\ \hline
% \textbf{Multi-domain utterance}       & 0            & 0              & 0              & \textbf{408}     \\ \hline
\textbf{Sentences}             & 248  & 2,912  & 17,181  & \textbf{71,425}  & \textbf{11,198}\\
\textbf{Avg. sentence length}  & 4.49 & 7.48   & 6.93    & \textbf{12.34}   & \textbf{11.00}\\
\textbf{Distinct Unigrams} & 96   & 2,182  & 3,007   & \textbf{4,458}  & \textbf{868} \\
\textbf{Distinct Bigrams}  & 218  & 4,004   & 21,997  & \textbf{39,340} & \textbf{4,089} \\
\textbf{Distinct Trigrams}  & 250  & 5,703  & 40,184  & \textbf{114,937} & \textbf{7,111}\\
\hline

\end{tabular}
}\label{tab:data_lexical}
\end{table}

==> temp.tex/text.tex <==

% Although some studies try to perform DST in the audio domain, their approaches are centered on ASR adoption. Thus, there is limited exploration of E2E models that utilize audio signals directly. In contrast, the related task of Spoken Language Understanding (SLU) investigates both E2E and ASR approaches to deal with user intent in utterances . However, SLU inputs comprise just simple single-turn user commands, and thus lack the comprehensive system context required for DST dialogues. In this study, not only do we extend the DST task to the audio paradigm by leveraging ASR, but we also incorporate an E2E model in order to directly utilize audio inputs.

% \noindent
% \newline
% \textbf{Leveraging Synthetic Data}
% The utilization of TTS synthetic data showed encouraged outcomes in replacing or supplementing human voice datasets within low-resource environments. Synthetic data has proven beneficial in speech recognition by enhancing system accuracy through self-training with synthesized data \cite{Related-self}, leveraging unpaired raw text \cite{Related-unpair}, and aiding in the comprehension of out-of-vocabulary words \cite{Related-oov}. In keyword spotting research, diversely styled synthetic data helped to find the target words \cite{Related-style}. Additionally, synthetic utterances generated from the prosody-aware TTS model have improved on-device punctuation prediction using \textbf{ [Find papers]. Nevertheless, no prior studies have explored the impact of synthetic data on DST research. Building upon previous successes, we undertook an investigation of the synthesized dataset's effect on audio modality DST. 




% Research in DST predominantly revolves around the text modality, which stems from the assumption that the upstream ASR models would provide error-free transcriptions of the speech utterances. However, this perspective overlooks a crucial aspect; there are inherent dissimilarities between spoken and text-based conversations, specifically in the inclusion of pronunciation variations that deviate from the presumed accurate text transcriptions. Recognizing the importance of addressing speech disfluencies, some studies have explored the utilization of the N-best ASR hypotheses \cite{Related-ASR1, Related-ASR2}. This approach leverages the collective power of multiple hypotheses, operating under the assumption that they possess the ability to complement one another, which then enhances language understanding capabilities. 

% Another avenue of research explores the integration of insights from diverse domains. For example, by taking advantage of the advancements in speech synthesis, some studies employ fine-tuning techniques to enhance Automatic Speech Recognition (ASR) models through the utilization of synthetic speech data \cite{Related-DataAug1, Related-DataAug2}. This approach aims to improve transcription prediction accuracy, particularly within specific domains. Additionally, other integrate word confusion networks to effectively model ASR ambiguity \cite{Related-wordconfusion}, which contributes to the development of more robust DST models that can effectively handle speech inputs. Furthermore, other investigations employ postprocessing methodologies \cite{Related-postprocessing} to address transcription errors originating from the ASR process.

% Moreover, the absence of consideration for noisy speech inputs in DST datasets, which are predominantly collected in text format, necessitates additional measures to bridge the gap between written and spoken conversations. To address this disparity, certain studies have explored the application of data augmentation techniques by introducing noise to the data to enhance the robustness of DST systems against spoken inputs while accounting for speech disfluency \cite{Related-DataAug1, Related-DataAug2}. Other studies utilize N-best ASR hypotheses as a means to leverage complementary information to facilitate better language understanding \cite{Related-ASR1, Related-ASR2}.
% % [some works add asr noise in order to make more speech ]



% Further quantitative and lexical statistics of SynthWOZ and human authentic test sets are in Tables~\ref{tab:data_audio} and \ref{tab:data_lexical}.

% To test the quality of our AudioWOZ synthetic and actual human speech, we use a pretrained Whisper model \cite{Whisper}, which is one of the state-of-the-art ASR systems trained on multilingual web data. The accuracy of the resulting ASR transcriptions are calculated via Word Error Rate (WER) and Character Error Rate (CER), and the results summarized in Table~\ref{tab:human_test_ASR} show minor pronunciation errors in both AudioWOZ's synthetic (i.e., \textit{Train, Dev, Test}) and human speech (i.e., \textit{Test-Human}) datasets. We also test AudioWOZ with Wav2Vec 2.0 (W2V) \cite{w2v}, which is another SOTA ASR model.

% \subsection{Quantitative Comparison with Other Datasets} 

% In Tables 3 and 4, we conduct quantitative and lexical analyses between our AudioWOZ dataset and other benchmark speech datasets used in other tasks (e.g., SLU) \cite{FSC, SNIPS, SLURP}. Compared to the largest SLU SLURP dataset, our AudioWOZ corpus is twice as big in terms of duration and in the number of audio files (Table 3). Moreover, as can be seen in Table 4, the proposed AudioWoz dataset boasts a natural dialogu e style with longer, more complex sentences, as evidenced by its higher number of sentences with longer average length. Additionally, its greater occurrence of distinct unigrams, bigrams, and trigrams appearing only once highlight greater lexical diversity and naturalness. With the presence of multi-intents in utterances and greater turn spans per intent, AudioWoz offers a more realistic dialogue structure, making it a highly accurate and representative dataset for human-machine interaction.

% In Tables~\ref{tab:data_audio} and \ref{tab:data_lexical}, we conduct lexical and audio analyses between our AudioWOZ dataset and other benchmark speech datasets. As this is the first speech dataset for S-DST, there are no directly comparable datasets. As such, we compare AudioWOZ with datasets used in the task of Spoken Language Understanding (SLU)\cite{FSC, SNIPS, SLURP}, as both S-DST and SLU aim to accomplish a user's goal through speech. Compared to the largest SLU dataset (SLURP), our AudioWOZ corpus is twice as big in terms of duration and in the number of audio files (Tables~\ref{tab:data_audio}). Moreover, in Table~\ref{tab:data_lexical}, the proposed AudioWoz dataset boasts a natural dialogue style with longer, more complex sentences, as evidenced by its higher number of sentences with longer average length. Additionally, its greater occurrence of distinct unigrams, bigrams, and trigrams highlight greater lexical diversity and naturalness. With the presence of multi-intents in utterances and greater turn spans per intent, AudioWoz offers a more realistic dialogue structure, making it a highly accurate and representative dataset for human-machine interaction.
%In Tables~\ref{tab:data_audio} and \ref{tab:data_lexical}, we conduct quantitative and lexical comparison between our AudioWOZ dataset and other benchmark speech datasets. Since this is the first speech dataset for S-DST, there are no directly comparable datasets. As such, we compare AudioWOZ with datasets used in the task of Spoken Language Understanding (SLU)\cite{SLURP, SNIPS, FSC}, as both S-DST and SLU aim to accomplish what a user expects of the system through speech. Compared to the largest SLU dataset (i.e., SLURP), our AudioWOZ corpus is twice as big in terms of duration and in the number of audio files (Table~\ref{tab:data_audio}). Moreover, in Table~\ref{tab:data_lexical}, the proposed AudioWoz dataset boasts a natural dialogue style with longer, more complex sentences, as evidenced by its higher number of sentences with longer average length. Additionally, its greater occurrence of distinct unigrams, bigrams, and trigrams highlight greater lexical diversity and naturalness. With the presence of multi-intents in utterances and greater turn spans per intent, AudioWoz offers a more realistic dialogue structure, making it a highly accurate and representative dataset for human-machine interaction.
% Tables~\ref{tab:data_audio} and \ref{tab:data_lexical} present a quantitative and lexical evaluation of our SynthWOZ dataset compared to other benchmark speech datasets. Since this is the first speech dataset designed for the S-DST task, there are no directly comparable datasets available. As such, we compare AudioWOZ with datasets that are used in the SLU task \cite{SLURP, SNIPS, FSC}, as both S-DST and SLU aspire to meet user objectives through speech interaction. Compared to the largest SLU dataset (SLURP), our AudioWOZ corpus is twice as big in terms of duration and number of audio files (Table~\ref{tab:data_audio}). Moreover, in Table~\ref{tab:data_lexical}, the proposed AudioWOZ dataset comprises a natural dialogue style with longer and more complex sentences, as evidenced by its higher number of sentences with longer average lengths. Additionally, its greater occurrence of distinct unigrams, bigrams, and trigrams highlights greater lexical diversity and naturalness. Since each dialogue consists of multiple turns and multiple turn spans per dialogue topic (i.e., the domains in AudioWOZ, and the intents in SLU datasets), AudioWOZ offers a more realistic dialogue structure, making it a highly accurate and representative dataset for human-machine interaction. A recent concurrent work\footnote{https://dstc11.dstc.community/} does consider audio input, but they first convert disfluent speech into text and then concentrate solely on improving cascading model performance while using inaccurate text transcriptions.




% \begin{table}[t]


% \centering
% \caption{Quantitative comparison of different speech-based datasets. \textit{Ours-S}: Synthetic, \textit{Ours-H}: Human Speech.}
% % \scalebox{0.76}{
% % \resizebox{\columnwidth}{!}{
% \begin{tabular}{l|c|l}
% \hline
% \multicolumn{1}{c|}{\textbf{}} & \textbf{Ours-S}    & \textbf{Ours-H} \\ \hline
% Audio Files                         & \textbf{142,850} & \textbf{1,018}  \\
% Duration {[}hrs{]}                 & \textbf{147.8}   & \textbf{1.27}  \\
% Avg. length {[}s{]}            & \textbf{3.7}     & \textbf{4.5} \\
% \hline
% \end{tabular}
% % }
% \label{tab:data_audio}
% \end{table}



% \begin{table}[t]
% \label{tab:data_lexical}

% \centering
% \caption{Lexical analysis of different speech-based datasets. \textit{Ours-S}: Synthetic, \textit{Ours-H}: Human speech.}
% % \resizebox{\columnwidth}{!}{
% \begin{tabular}{l|l|l}
% \hline
% &  \textbf{Ours-S} & \textbf{Ours-H} \\ \hline
                                          
% \textbf{Sentences}             & 71,425  & 11,198\\
% \textbf{Avg. sentence length}    &12.34   & 11.00\\
% \textbf{Distinct Unigrams}    &4,458  & 868 \\
% \textbf{Distinct Bigrams}    & 39,340&4,089 \\
% \textbf{Distinct Trigrams}  &114,937 & 7,111\\
% \hline

% \end{tabular}
% % }
% \label{tab:data_lexical}
% \end{table}


